Is CADP an Applicable Formal Method?

CADP is a comprehensive toolbox implementing results of concurrency theory. This paper addresses the question, whether CADP qualifies as an applicable formal method, based on the experience of the authors and feedback reported by users.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{M. Gleirscher, J.v.d. Pol, J. Woodcock (Eds.):\\First Workshop on Applicable Formal Methods (AppFM 2021).\\
EPTCS 349, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.349.1}{10.4204/EPTCS.349.1}}

